Echo: KV-Cache-Free Associative Recall with Spectral Koopman Operators

Long chain-of-thought reasoning and agentic tool-calling produce traces spanning tens of thousands of tokens, yet Transformer KV caches grow linearly with sequence length, creating a memory bottleneck on commodity hardware. State-space models offer constant-memory recurrence but suffer a memory cliff: retrieval accuracy collapses once the gap between a stored fact and its query exceeds the effective horizon of the recurrent state. We introduce Echo, a KV-cache-free associative recall architecture built around Spectral Koopman Attention (SKA); a drop-in replacement for attention layers that augments SSM blocks with a closed-form dynamical operator whose sufficient statistics are accumulated in constant memory with no KV cache. Echo fits a spectral linear system to the key and value history via kernel ridge regression and retrieves through a learned power-iterated filter, all from $O(r^{2})$ streaming state where $r$ is a small projection rank. On the Multi-Query Associative Recall benchmark, a pure Mamba-2 SSM fails to exceed chance accuracy (${\sim}3\%$) across all gap lengths and KV-pair counts, while at the 50M parameter scale SKA-augmented models achieve $100\%$ retrieval accuracy on every configuration tested, including distractor gaps of $4{,}096$ tokens with $32$ KV pairs. Across five additional transfer benchmarks including needle-in-a-haystack, tool-trace, and multi-hop retrieval, SKA consistently outperforms both pure SSM and SSM+Attention hybrids while maintaining constant inference memory. Ablations confirm that the spectral operator, not the prefix masking strategy, drives the retrieval gain.

==> figures/50m_mqar_heatmap.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{assets/mqar_heatmap_intask.png}
    \caption{In task MQAR}
    \label{fig:MQAR_heatmap}
\end{figure}

==> figures/synthetic_experiments.tex <==
\begin{figure*}
    \centering
    \textbf{Zero-Shot Retrieval Transfer Across Architectures}\par\medskip
    \begin{subfigure}[ht!]{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/niah_transfer.png}
        \caption{Needle-in-a-haystack}
        \label{fig:niah}
    \end{subfigure}
    \vspace{0.5em}
    \begin{subfigure}[ht!]{1.0\linewidth}
        \centering
        \includegraphics[width=\linewidth]{assets/multihop_transfer.png}
        \caption{Two-hop retrieval}
        \label{fig:multihop}
    \end{subfigure}
    \caption{Zero-shot retrieval accuracy vs.\ sequence length and KV count for single-hop (a) and two-hop (b) tasks. The pure SSM degrades sharply at longer sequences; SSM+Attn improves but still drops; SSM+SKA (982K params) maintains the highest accuracy and flattest profile across all settings.}
    \label{fig:transfer-retrieval}
\end{figure*}

==> figures/synthetic_multihop_transfer.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{assets/multihop_transfer.png}
    \caption{\textbf{Zero-Shot Multi-Hop Retrieval Transfer Across Architectures.} Two-hop retrieval accuracy as a function of sequence length and number of key-value pairs. The pure SSM (left) fails to exceed 60\% even at short sequences and collapses toward chance at length 256, indicating that compositional retrieval compounds the memory decay observed in single-hop tasks. SSM+Attn (center) substantially improves over the pure SSM but shows sensitivity to KV count at longer sequences. SSM+SKA (right) achieves the highest accuracy across all settings and exhibits the most graceful degradation, suggesting that SKA's length-independent sufficient statistics benefit multi-hop reasoning as well as single-hop retrieval.}
    \label{fig:Multi_hop}
\end{figure}

==> figures/synthetic_niah_transfer.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{assets/niah_transfer.png}
    \caption{Needle in a haystack tasks}
    \label{fig:NIAH}
\end{figure}

==> sections/4.1-old.tex <==
\subsection{Resource Economy}
\label{sec:exp_economy}

The Resource Economy task tests whether SKA can track
cumulative state dynamics with conservation laws, going beyond
single-step associative recall to multi-step reasoning over
latent variables.

\paragraph{Task.}
A set of agents operate in a token economy with two resources
(gold and wood).
At each timestep an agent performs one of four actions:
\emph{mine} (increment a resource by 1--3),
\emph{build} (decrement one or both resources),
\emph{trade} (transfer a quantity from one agent to another,
conserving the total), or
\emph{rest} (no-op).
The episode is encoded as a pipe-delimited action log, e.g.\
\texttt{A+2g|B>A1w|C-1g2w|...}.
After the action sequence, and optionally a noise gap of
irrelevant chatter tokens, a query asks for a specific agent's
current count of a specific resource.
The answer is a two-digit zero-padded integer.
Resource counts are clamped to $[0, 99]$.

\paragraph{Relevance to Koopman analysis.}
Trades conserve total resources across agents, creating a
persistent eigenmode ($|\lambda| \approx 1$) in the latent
dynamics.
Mining and building change totals, producing transient modes.
The Koopman operator's eigenspectrum should separate these:
persistent modes encode conservation laws that must survive
the noise gap, while transient modes can be safely suppressed
by the power filter.

\paragraph{Tiers.}
We use two difficulty levels:
\begin{itemize}
    \item \textbf{Easy}: 5--15 action steps, 3 agents, no noise
          gap. The horizon is short enough that SSM state
          retention is not challenged.
    \item \textbf{Hard}: 40--100 action steps, 6 agents,
          200--400 tokens of noise gap injected between the
          action log and the query.
          The combination of a long action sequence and a
          substantial noise gap forces the SSM's continuous state
          to decay before query time.
\end{itemize}
Both tiers are trained for 2{,}500 steps with batch size 16.
The action mask marks only the action-log tokens, excluding
the noise gap.

\paragraph{Memory cliff analysis.}
We report the accuracy drop from Easy to Hard for each model.
A large drop indicates a memory cliff: the model solves the
task when the horizon is short but fails when cumulative state
must be preserved across a noise gap.
